Inter-Session Modeling for Session-Based Recommendation

In recent years, research has been done on applying Recurrent Neural Networks (RNNs) as recommender systems. Results have been promising, especially in the session-based setting where RNNs have been shown to outperform state-of-the-art models. In many of these experiments, the RNN could potentially improve the recommendations by utilizing information about the user's past sessions, in addition to its own interactions in the current session. A problem for session-based recommendation, is how to produce accurate recommendations at the start of a session, before the system has learned much about the user's current interests. We propose a novel approach that extends a RNN recommender to be able to process the user's recent sessions, in order to improve recommendations. This is done by using a second RNN to learn from recent sessions, and predict the user's interest in the current session. By feeding this information to the original RNN, it is able to improve its recommendations. Our experiments on two different datasets show that the proposed approach can significantly improve recommendations throughout the sessions, compared to a single RNN working only on the current session. The proposed model especially improves recommendations at the start of sessions, and is therefore able to deal with the cold start problem within sessions.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand


